Constrained Mixture Models for Asset Returns Modelling

The estimation of asset return distributions is crucial for determining optimal trading strategies. In this paper we describe the constrained mixture model, based on a mixture of Gamma and Gaussian distributions, to provide an accurate description of price trends as being clearly positive, negative or ranging while accounting for heavy tails and high kurtosis. The model is estimated in the Expectation Maximisation framework and model order estimation also respects the model's constraints.

==> constrainedmixturemodels copy/userdefs.tex <==

% frequently used environments
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\bean}{\begin{eqnarray*}}          % not numbered equation
\newcommand{\eean}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bt}{\begin{tabular}}
\newcommand{\et}{\end{tabular}}
\newcommand{\bfig}{\begin{figure}[htb]}
\newcommand{\efig}{\end{figure}}

\newcommand{\cl}{\centerline}
\newcommand{\dstyle}{\displaystyle}

% frequently used styles
\newcommand{\Bs}[1]{\boldsymbol{#1}}
\newcommand{\vs}{\vspace{2cm} \noindent}
\newcommand{\ul}{\underline}
\newcommand{\bm}[1]{\mbox{\boldmath $#1$}}
\newcommand{\mc}[1]{{\mathcal{ #1}}}
\newcommand{\hicite}[1]{$^{\cite{#1}}$}

% frequently used fractions
\renewcommand{\d}[2]{\frac{d #1}{d #2}}
\newcommand{\pD}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dd}[2]{\frac{d^2 #1}{d {#2}^2}}
\newcommand{\DD}[2]{\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\Dmix}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3 }}

% frequently used symbols
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Sig}{\mbox{\boldmath $\Sigma$}}
\newcommand{\Gauss}[1]{\mathcal{N}(#1)}
\newcommand{\Wi}{{\mathcal W}}
\newcommand{\Dir}{{{\mathcal D}ir}}
\newcommand{\MvN}{{{\mathcal M}v{\mathcal N}}}
\newcommand{\Ga}[1]{{\mathcal Ga}(#1)}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\inv}{^{\mathsf{-1}}}
\newcommand{\invt}{^{\mathsf{-T}}}
\newcommand{\pinv}{^{\mathsf +}}
\newcommand{\pinvt}{^{\mathsf{+T}}}
\newcommand{\tp}{^{\mathsf T}}
\newcommand{\defeq}{\stackrel{\tiny \mathrm{def}}{=}}
\newcommand{\etr}{\mbox{etr}}
\newcommand{\tr}{\mathrm{tr}}

\newcommand{\Alpha}{{A}}
\newcommand{\Beta}{{B}}

\newcommand{\bvec}[1]{\vec{\mbox{\boldmath $#1$}}}
\newcommand{\vcg}[1]{\mbox{\boldmath $#1$}}
%\newcommand{\bm}[1]{\mbox{\boldmath $#1$}}
%\newcommand{\inv}{^{-1}}
%\newcommand{\mc}[1]{{\mathcal #1}}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\eqnref}[1]{(\ref{#1})}
\newcommand{\figref}[1]{(\ref{#1})}


